Emergent Cooperative Behavior in Distributed Target Tracking with Unknown Occlusions

Tracking multiple moving objects of interest (OOI) with multiple robot systems (MRS) has been addressed by active sensing that maintains a shared belief of OOIs and plans the motion of robots to maximize the information quality. Mobility of robots enables the behavior of pursuing better visibility, which is constrained by sensor field of view (FoV) and occlusion objects. We first extend prior work to detect, maintain and share occlusion information explicitly, allowing us to generate occlusion-aware planning even if a priori semantic occlusion information is unavailable. The efficacy of active sensing approaches is often evaluated according to estimation error and information gain metrics. However, these metrics do not directly explain the level of cooperative behavior engendered by the active sensing algorithms. Next, we extract different emergent cooperative behaviors that stem from the same underlying algorithms but manifest differently under differing scenarios. In particular, we highlight and demonstrate three emergent behavior patterns in active sensing MRS: (i) Change of tracking responsibility between agents when tracking trajectories with divergent directions or due to a re-allocation of the resource among heterogeneous agents; (ii) Awareness of occlusions to a trajectory and temporal leave-and-return of the sensing agent; (iii) Sharing of local occlusion objects in MRS that subsequently improves the awareness of occlusion.

==> slides/behavior.tex <==

\begin{frame}{Visibility}
    Visibility: the object $t$ is \textit{visible} to robot $i$ at time $k$ if and only if $t$ is inside the FoV and not in any occlusion area; the set of visible objects to robot $i$ is defined
    \begin{equation}
        \label{eq:visibility}
        \mathcal{V}_{i, k} = \{t| (\chi_{t, k} \in \phi_{i, k}) \land (\chi_{t, k} \notin W)  \},
        % \mathcal{V}(t, i) = \left\{ z | \left(\mathbf{z}_{t, i} \in \phi_i(s) \right) \land \left(\mathbf{z}_{t, i} \notin W \right) \right\}
    \end{equation}
and the visible objects to the team is $\mathcal{V}_{k} = \cup_{i \in [N]} V_{i, k}$.
\end{frame}

\begin{frame}{}
    \begin{definition}[\ownership$(i, t, k)$]
Robot $i$ obtains the \textit{m-Ownership} of the target $t$ at time step $k$ if robot $i$ detects $t$ for $m$ consecutive time steps, i.e., $\forall 0 \leq h \leq m, t \in \mathcal{V}_{i, k + h}$.
\end{definition}

    \begin{definition}
[\bhonwershipchange{i}{j}{t}]
The behavior \textit{Ownership\_Change} happens between robot $i, j$: at time step $0$ target $t \in M_{i, k} \land t \notin M_{j, k}$, and after $L$ steps the ownership goes to $j$, i.e., $t \in M_{j, k + L} \land t \notin M_{i, k + L}$.
\end{definition}
\end{frame}

\begin{frame}{Occlusion Aware}
   \begin{definition}[\textit{Occlusion\_Aware}$(k_0, t, W, L, h)$]
The OOI $t$ is occluded at all time steps $k \in [k_0 + h, k_0 + L-h], \chi_{t, k} \in W$.
We say the behavior is \textit{Occlusion\_Aware} with the satisfaction of all three conditions below.
\begin{enumerate} 
    \item $\exists S_1\subseteq [N]$, $S_1 \neq \emptyset$ s.t. $\forall i \in S_1$, $t \in M_{k_0, i}$;
    \item $\nexists i \in [N]$ s.t. $\forall k \in [k_0 + h, k_0 + L-h]$, $(M_{k, i} = \emptyset) \land (\chi_{t, k} \in \phi_{i, k})$;
    \item $\exists S_2\subseteq [N]$, $S_2 \neq \emptyset$ s.t. $\forall i \in S_2$, $t \in M_{k_0 + L, i}$;
\end{enumerate}
\end{definition}
\end{frame}

\begin{frame}{Occlusion Sharing}
    \begin{definition}[\textit{Occlusion\_Sharing}]
Define an \textit{occlusion-detection event} $e$ as an occlusion $w \in W$ is detected by robot $i$ at time step $k$, i.e. $e = \{w \in \phi_{i, k}\}$, then $\forall h > k$ and any trajectory $t$.

The definition of \occlusionshare\ is loosely based on the probability of behavioral event \occlusionaware\ in the future, 
\begin{equation}
    \label{eq:occlusion-share}
    \mathbb{P}[\textit{OA}(t, W_h, L, h) | e] \geq \mathbb{P}[\textit{OA}(t, W_h, L, h)],
\end{equation}
where the term \textit{OA} is the abbreviation of \occlusionaware. 
\end{definition}
\end{frame}

==> texts/numerical_result.tex <==

\section{Numerical Result}
\label{sec:result}


\textit{Trajectory Handover}: the initial ownership is $M_0 = {}$

\begin{figure}
    \centering
    \includegraphics[width = .5\textwidth]{pics/sankey_trajhandover.png}
    \caption{Sankey plot of the ownership change in Trajectory Handover case. From top to bottom the algorithms are: SMA-NBO, PMA-NBO, Dec-POMDP-NBO.}
    \label{fig:my_label}
\end{figure}


\textit{Resource Allocate}: the initial ownership is $M_0 = {}$

\begin{figure}
    \centering
    \includegraphics[width = .5\textwidth]{pics/sankey_resourceallocate.png}
    \caption{Sankey plot of the ownership change in Resource Allocate case. From top to bottom the algorithms are: SMA-NBO, PMA-NBO, Dec-POMDP-NBO.}
    \label{fig:my_label}
\end{figure}

==> texts/related_works.tex <==
\section{Related Works in Active Sensing}

With the development of reasoning and robotics, sensing is a task more than just passively processing the signal.
Mobility enables the sensing agents to improve the sensors' field of view (FoV), and prediction and inference support sensing in reasoning motions with a higher chance of detection and better data quality.
Such sensing-oriented autonomous system is widely studied and applied in rescuing \cite{mobedi20113}, event recording and analysis \cite{wu2019interactive, shell2019planning},
surveillance and monitoring, etc.

However, sensing is always full of difficulty since the problem of FoV and 

In this paper, we study the approach to better active sensing via the semantic information of the environments.
The impact of occlusion to general sensors are critical: in some scenario such occlusion can be avoided by a better sensing position (paper); however, there are cases sensing agents must accept the occlusion and balance all sensing objects.

Given a map, a good plan can be made like \cite{li2022sma}.

Such map is not always available. 
In this paper, we propose a cooperative active sensing in target tracking scenarios in the environment with unknown sensing.

\subsection{Active Sensing}

Active sensing, is a pattern of behavior in intelligent agents which \cite{yang2016theoretical}.
There are two main components in active sensing: perception and action. 
The perception component processes the information from sensor and maintains the belief of the environment;
action component generates response to information gathered so far, and optimize the future sensing.

% active sensing's task and areas
The extension of active sensing to robotics,
active cooperative perception \cite{spaan2010active},
information-driven control,...
% applications, SLAM, detection


\subsection{Sensing with Occlusion}

\cite{bernreiter2019multiple} semantic in SLAM

From detection side
\cite{lu2021global} occlusion with moving targets
local and global integration tracking (LGIT) \cite{yao2022semantic}

From data association side
\cite{ur2015multi} in JPDA framework, scenario of multi-target with complex occlusion.
\cite{chen2019multi} studies the multi target tracking with semantics, S-PHD filter.

Motivation
from planning/control side, in a non-myopic 
\begin{itemize}
    \item \cite{jung2002tracking} visibility maximization in a complex environment with occlusions, area can be divided by FoV of robots.
    \item \cite{bandyopadhyay2009motion} defines a POMDP with loosely control in an occupancy discrete world, to reduce of uncertainty of human position with allowing target outside of FoV (single agent).
    \item \cite{jakob2010occlusion} occlusion consideration in urban environment, with the objective of minimizing the \textit{information age} of all target area.
    \item \cite{bhattacharya2011cell, zou2018optimal} models the tracking problem in environments with occlusions and solves the planning problem via game theoretic model.
    \item \cite{hausman2016occlusion} occlusion of other robots in a UAV-fleet.
    \item \cite{nageli2017real} optimizes the viewpoint of a single UAV's camera in human detecting via receding horizon MPC
    \item \cite{tallamraju2019active} measures the multi-object tracking with static occlusion (trees).
    \item \cite{lopez2019adaptive} a circular formation of multi-UAV tracking 1 targets with constraint of FoVs.
    
\end{itemize}
% \cite{jung2002tracking} visibility maximization in a complex environment with occlusions, area can be divided by FoV of robots.
% \cite{bandyopadhyay2009motion} defines a POMDP with loosely control in an occupancy discrete world, to reduce of uncertainty of human position with allowing target outside of FoV (single agent).
% \cite{bhattacharya2011cell} models the tracking problem in environments with occlusions and solves the planning problem via game theoretic model.
% \cite{hausman2016occlusion} occlusion of other robots in a UAV-fleet.
% \cite{tallamraju2019active} measures the multi-object tracking with static occlusion (trees).

previous work has investigated the active sensing with semantic map of the environment; and we are considering the condition that the ground truth semantic map is not available: a fleet of UAVs are detecting in a strange area where they have no prior semantic information. 
In this case, the UAVs are simultaneously recognizing the occlusions via sensors, updating the local occlusion, sharing/maintaining local occlusion detection, and planning based on local occlusion maps.
